Supporting Software Maintenance with Dynamically Generated Document Hierarchies

Software documentation supports a broad set of software maintenance tasks; however, creating and maintaining high-quality, multi-level software documentation can be incredibly time-consuming and therefore many code bases suffer from a lack of adequate documentation. We address this problem through presenting HGEN, a fully automated pipeline that leverages LLMs to transform source code through a series of six stages into a well-organized hierarchy of formatted documents. We evaluate HGEN both quantitatively and qualitatively. First, we use it to generate documentation for three diverse projects, and engage key developers in comparing the quality of the generated documentation against their own previously produced manually-crafted documentation. We then pilot HGEN in nine different industrial projects using diverse datasets provided by each project. We collect feedback from project stakeholders, and analyze it using an inductive approach to identify recurring themes. Results show that HGEN produces artifact hierarchies similar in quality to manually constructed documentation, with much higher coverage of the core concepts than the baseline approach. Stakeholder feedback highlights HGEN's commercial impact potential as a tool for accelerating code comprehension and maintenance tasks. Results and associated supplemental materials can be found at https://zenodo.org/records/11403244

==> format.tex <==
\usepackage[T1]{fontenc}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{xcolor}
\usepackage{url}
\usepackage{array}
\usepackage{color}
\usepackage{wasysym}
\usepackage{verbatim}
\usepackage{bigstrut}
\usepackage{multirow}
\usepackage{setspace}
\usepackage{tabularx}
\usepackage{xspace}
\usepackage{subcaption}
\usepackage[font=footnotesize]{caption}
\usepackage{soul}
\usepackage{vcell}
\usepackage{pifont}
\usepackage{afterpage}
\usepackage{rotating}

\usepackage{graphicx}
\usepackage{enumitem}

\usepackage{balance}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{algpseudocode}
\usepackage{hyperref}
\usepackage{ulem}
\usepackage{amssymb}
\usepackage{wrapfig}
\usepackage{tcolorbox}

\newcommand{\jch}[1]{{\textcolor{blue}{#1}}} %blue
\newcommand{\kd}[1]{{\textcolor{red}{#1}}} %red

\definecolor{dkgreen}{HTML}{006400}
\newcommand{\ar}[1]{\textcolor{dkgreen}{#1}} %green

==> notes/gpt_as_evaluator.tex <==
% As noted earlier, metrics like BLEU and ROUGE are standard for comparing machine-generated content to developer-created versions; however, they don't capture all the nuances of multi-layer documentation. Further, they have demonstrated weak correlation with human evaluations, particularly for documentation of average quality \cite{Hu_Chen_Wang_Xia_Lo_Zimmermann_2022, Liguori_Improta_Natella_Cukic_Cotroneo_2023}. Interestingly, GPT-3 and GPT-4 models have shown the highest correlation with human evaluations in NLG \cite{Wang_Liang_Meng_Sun_Shi_Li_Xu_Qu_Zhou_2023, Fu_Ng_Jiang_Liu_2023, Liu_Iter_Xu_Wang_Xu_Zhu_2023}, though they tend to favor outputs from large language models over human-written text \cite{Liu_Iter_Xu_Wang_Xu_Zhu_2023}. We incorporate results from both project experts and GPT-4, but we base our conclusions solely on the input from the project experts. The inclusion of GPT-4 scores is primarily intended to assess how its judgments compare to those of the experts. This evaluation helps us determine the potential utility of GPT-4 for future research, especially in situations where expert input is not readily available.

==> sections/future-work.tex <==
% Although HGEN marks a step forward toward production-grade documentation, there are several areas which warrant further exploration to maximize the usefulness of the documentation. As highlighted in Section \ref{sec:artifact_quality}, the structure of the hierarchy often differs from how the expert's think about their code. This underscores the subjective nature of documentation which can be formed based on different attributes of the code (e.g. feature vs architecture). Currently, the clustering process in HGEN only supports direct semantic comparisons and does not allow for customized groupings focused on multiple aspects. To address this, we have begun a preliminary investigation into integrating user goals into the clustering process, allowing the groupings to be formed around the attribute most critical to a specific user or project. In addition, we are exploring the use of integrating Abstract Syntax Trees (ASTs) to improve the creation of meaningful clusters that encapsulate aspects beyond the code semantics. Finally, we are exploring different size clusters to achieve a wider range of project goals, such as using larger clusters to extract high-level system overviews instead of detailed system-level implementations.

% Another area for future development is the dynamic updating of documentation as the system evolves. Establishing relationships during the HGEN process lays a groundwork for identifying related documents that need updated when a change occurs. However, the best way to automatically facilitate these updates, remains an interesting area for future exploration.

Our future work with HGEN is aimed at enhancing its automated documentation capabilities through several key improvements. We plan to refine the clustering mechanism by incorporating user-specific goals, facilitating the creation of documentation that aligns with diverse code attributes like features or architecture. This includes exploring the integration of Abstract Syntax Trees (ASTs) to generate more comprehensive clusters. Furthermore, we are examining the use of varied cluster sizes to cater to a range of project needs, from high-level overviews to detailed implementations. Another critical area of development is enabling dynamic updates in response to system changes, leveraging the relationships established by the trace links. This advancement will ensure the continuous relevance and accuracy of documentation throughout the software development lifecycle, marking a significant stride in the field of automated documentation.

==> sections/motivation.tex <==

Our initial investigations into the use of LLMs to generate documentation started very simply. We attempted to leverage Anthropic’s claude-2.0 \cite{claude}, chosen due to its 100k-token context window,  and provided \emph{all} source code or low-level artifacts into a \emph{single} prompt along with the instructions to generate the intended higher-level software artifacts. This provided a baseline for the language model's unaided performance. However, our discussions with software engineers revealed that this approach fell short in the following ways:

\begin{enumerate}
    \item It provided no clear groupings of related functionality.
    \item The features were specified at a broad level of granularity.
    \item The model only covered the core features of the code base.
    \item Significant effort was required to review predicted trace links.
\end{enumerate}

While the off-the-shelf large language model showed initial promise, these critiques highlighted several deficiencies that would need to be addressed before the system could be deployed for industrial applications. As a result, our present methodology was devised with the primary objective of addressing the shortcomings of the baseline approach. 

==> sections/results.tex <==










==> sections/roadmap.tex <==
% Research roadmap

In this paper, we have proposed HGEN as a novel approach that not only seeks to generate software artifacts but also their associated trace links from source code. Our experimental validation has shown the promise of the approach but has also revealed areas that need improvement. To encourage other researchers to enter this field, we layout an initial research roadmap listing six open challenges [C1-C6] identified through our study. 

\begin{itemize}[leftmargin=.1em]
  \setlength\itemsep{.5em}
    \item []{\bf C1: Improved Duplication Detection} \vspace{2pt}\\
One of the greatest needs for improvement is the better detection and elimination of duplicate artifacts, as highlighted in Section \ref{sec:uniquness}. As observed, many duplicate artifacts currently remain undetected. Enhancing the vector representations of generated artifacts, either through improved embedding models or by fine-tuning on specific projects, could strengthen duplicate detection capabilities. Additionally, exploring techniques to create more distinct clusters in Step 1 of the HGEN process may reduce duplicates by avoiding the generation of highly similar artifacts in the first place. Tackling this challenge could lessen the manual review burden on engineers and enable better separation of features. 

  \item []{\bf C2: Increasing Artifact Granularity} 
  \vspace{2pt}\\
  An additional problem encountered was that some of the lower-level documentation consolidated too many features into a single artifact, resulting in an artifact that was harder to verify, as discussed in Section \ref{sec:feature_coverage}. Future work should target improved clustering strategies for decomposing groups of source code into finer levels of granularity, thus producing more focused and detailed documentation at the initial layer. 

  \item []{\bf C3: Interactive and Iterative Process} 
  \vspace{2pt}\\ The current HGEN process automated the generation of the entire artifact hierarchy. However, it could be beneficial to adapt it so that users can customize their own inputs, tailoring the process for specific projects or use-cases. One area where user input could yield significant benefits is the clustering process. Future research may explore methods to integrate user preferences, such as the separation of CRUD operations (as discussed in Section \ref{sec:amlgamation}), into the clustering process.
  
  Likewise, providing interactive tools that empower users to approve or decline generated artifacts, or to prompt the model to modify specific elements within an artifact, would likely be needed for HGEN's adoption across more diverse domains. The challenge is, therefore, to transform the process into a more interactive one, enabling engineers to align the output more closely with their own objectives.


\item []{\bf C4: Documentation Completion} 
\vspace{2pt}\\
Presently, HGEN is restricted to the creation of a complete layer of documentation where none currently exists. However, there is real potential for using HGEN to augment or even to validate and evolve partially complete documentation. An open area for exploration is identifying optimal methods to recognize gaps in existing documentation and efficiently supplement those gaps. This could enable focused generation to fill in missing documentation pieces, rather than only creating new layers. It could also facilitate an automatically evolving artifact tree, where system updates are immediately reflected in existing documentation.

\item []{\bf C6: Community Benchmarks} 
\vspace{2pt}\\
Finally, as a meta-challenge, we need to develop new benchmark datasets and associated metrics for assessing the quality of generated artifacts and artifact hierarchies. We contribute to this by sharing initial solutions for the two OSS (Dronology and JOC); however, we need better ways to quantitatively and qualitatively compare results, and additional benchmark datasets. 
\end{itemize}

% \begin{itemize}[leftmargin=.5em]
%     \item []{\bf C1: Clear Hierarchical Abstraction} \vspace{2pt}\\
%    One notable problem we observed in the HGEN documentation was that higher layers tended to replicate, rather than create new abstractions from lower layers. This observation was based on both participant discussions (Section \ref{sec:newcomer_results}) and the observation of roughly equal artifact numbers between the lower and higher levels (Table \ref{tab:projects}). The challenge is to {\bf generate hierarchies that consistently exhibit increased levels of abstraction and reduced redundancy at each ascending level.}
% \end{itemize}
% % \noindent{\it Potential Solutions:~}[C1.1] Introduce a "grouping" step, wherein the model is required to first cluster related child artifacts before generating the new documentation. This additional step may aid the model in identifying relationships and patterns in the child layer that would facilitate meaningful abstractions in the parent layer. 
% %  [C1.2] Modify prompts to prioritize this goal in the higher levels of the hierarchy and/or incorporate illustrative examples into the prompt.

% \subsection*{C2: Enriched Artifact Details} \vspace{2pt}
% \noindent Another challenge encountered in our work was the limited level of details generated for certain artifacts. This posed an obstacle for newcomers who were unfamiliar with the project, suggesting a need for additional information to effectively onboard new engineers. Moreover, as exemplified in the Dronology dataset, safety-aware systems demand more explicit details for safety verification and requirements validation purposes. Unfortunately, many of our attempts to increase the details in the artifacts resulted in an increased likelihood that the model would fabricate information  to compensate for its information gaps. The challenge is to {\bf create detailed artifacts without including hallucinations}. 
%  \vspace{3pt} \\
% \noindent{\it Potential Solutions:~} 
% [C2.1] A potential solution could involve partitioning the source code into meaningful chunks, allowing the model to concentrate on smaller areas of the system at a time. Subsequently, the model could either generate the parent artifacts from each chunk and consolidate the combined list of parents afterward, or create a detailed summary of each chunk for reference while generating all the parent artifacts at once. Initial experiments showed promise in the model's ability to extract additional details from smaller subsets of the code,  but it remains an open challenge of how best to automate the partitioning of the code. [C2.2] The input questions provided to Step 1 of the HGEN process could be refined to better assist the model in extracting the essential details during summary generation. This approach might be particularly well suited when the user possesses prior insights into the types of details crucial for inclusion in the artifacts. 

% \subsection*{C3: Increasing Artifact Granularity} \vspace{2pt}
% \noindent {\it Challenge Description:~} An additional problem encountered was that the documentation often consolidated too many features into a single artifact, resulting in an artifact that was very broad and thus harder to verify. This was particularly evident in the design descriptions of Dronology, as discussed in Section \ref{sec:feature_coverage}. It will be necessary for future work to devise strategies to encourage more granular artifacts, enabling concrete verification and establishing more focused traceability links.
% \vspace{3pt} \\
% \noindent{\it Potential Solutions:~} 
% [C3.1] Building on the observed success of instructing the model to adhere to specific criteria, a straightforward path forward could be to explicitly incorporate this constraint in the prompt.
% [C3.2] An alternative method could be to introduce a "refinement" step after artifact creation that encourages the model to decompose unnecessarily broad artifacts. Allowing the model to concentrate on this singlular task during the refinement phase might be simpler for the model than attempting to achieve it during the initial artifact creation.

% \subsection*{C4: Creating an Iterative Process} \vspace{2pt}
% \noindent {\it Challenge Description:~} The current HGEN process is fully automated such that most inputs are created solely by the model. However, the breakdown of the current process opens the possibility for users to develop their own input, tailoring the process for specific projects or use-cases. For instance, to ensure the inclusion of acceptance criteria, users could modify the format used in Step 2, as demonstrated in Section \ref{sec:formatting}. Additionally, incorporating more project-specific questions into Step 1's input could yield a more useful summary. Likewise, enabling users to approve or decline generated artifacts, or to prompt the model to modify specific elements within an artifact, will likely be necessary for HGEN's adoption across all domains, especially in safety-critical fields. Future work might transform the process into a more interactive one, enabling engineers to align the output more closely with their own objectives.

% \vspace{3pt} \\
% \noindent{\it Potential Solutions:~}  [C4.1] One approach is to develop an interface that presents users with the model's suggested input for the next step, enabling them to either approve, regenerate, or modify it.  This would grant users the flexibility to be as involved or uninvolved in the process as they desired. Furthermore, the interface should offer a way for users to provide feedback on generated artifacts which could be used to prompt the model to regenerate an improved version.

% \subsection*{C5: Filling in Missing Documentation} \vspace{2pt}
% \noindent {\it Challenge Description:~} 
% Presently, HGEN is restricted to the creation of a complete layer of documentation when none already exists. Yet, there is a potential use-case for automatic documentation generation, which involves filling information gaps in cases of missing or incomplete documentation. Future work could explore how to modify the process to effectively meet this need.

% \vspace{3pt} \\
% \noindent{\it Potential Solutions:~}  
% [C5.1] Addressing this demand may necessitate additional steps in the current process. Specifically, a step could be introduced that takes in the source code and existing documentation and tasks the model with identifying any functionality that currently lacks coverage. This output could then be integrated into the artifact generation phase, directing the model to focus on creating documentation exclusively for the missing functionality.

 

==> sections/traceability.tex <==

Using the trace links that were added, confirmed, or rejected by the project experts, we conducted a quantitative assessment of the traceability within the generated dataset, as shown in Table \ref{tab:tracing_results}. We deem robust traceability integral to the effectiveness of HGEN, as these trace links enable engineers to quickly identify code pertinent to particular features. Moreover, these links illuminate documentation requiring updates when associated system modifications occur, facilitating the evolution of the documents.

In addition to assessing the effectiveness of HGEN in capturing relationships, we aimed to compare post-process predictions with those generated during the HGEN process, wherein the original clusters were considered in the predictions. We report the results of the post-process predictions using both the Sentence-BERT embeddings and the Vector Space Model (VSM) technique, a widely used baseline in traceability research \cite{vsm}. With both approaches, we compute the similarity score for each potential pair of higher-level and lower-level artifact and deem any pairs with a score above 0.5 as a predicted link. By examining \emph{all} artifact pairs, predictions can be made between higher-level artifacts from different clusters than the initially associated lower-level artifacts.

Our evaluation employed multiple metrics, including mean average precision (MAP), precision, recall, and F2 score, where MAP assesses the method's ability to rank true positives effectively, and F2 represents a weighted harmonic mean of precision and recall, leaning toward recall.

Across the board, HGEN is able to retain high precision score ($>$80\%) while never dropping below 90\% recall. Further, the high MAP signals that the scores assigned to the predictions are reflective of the strength of the link. The relatively high performance of VSM is likely because HGEN generates the artifacts directly from the lower-level, reusing much of the same terminology, allowing semantic-based traceability approaches to excel at link predictions. 

The consensus among all experts was predominantly positive, as the experts felt the predicted traced links required very few revisions. JOC needed to decline 17 of 99 links and add no new links, Dronology declined 28 of 195 links and added 18 new ones, and SAFA declined only 5 of 81 links and added 8 new links.

\begin{table}[htbp]
    \centering
    \caption{Traceability Performance Metrics}
    \label{tab:tracing_results}
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Dataset} & \textbf{Method} & \textbf{MAP} & \textbf{Precision} & \textbf{Recall} & \textbf{F2} \\
        \midrule
        \multirow{2}{*}{SAFA} & Clustering & 94.7 & 93.8 & 90.5 & 92.1 \\
                              & Embeddings & 78.3 & 55.7 & 67.1 & 64.5 \\
                              & VSM        & 79.8 & 48.4 & 77.6 & 69.2 \\
        \midrule
        \multirow{2}{*}{Dronology} & Clustering & 97.8 & 85.6 & 90.3 & 87.9 \\
                                   & Embeddings & 75.8 & 19.1 & 85.3 & 50.4 \\
                                   & VSM        & 68.3 & 27.9 & 78.9 & 57.8 \\
        \midrule
        \multirow{2}{*}{JOC} & Clustering & 86.7 & 82.3 & 100 & 90.6 \\
                             & Embeddings & 75.0 & 73.8 & 59.6 & 62.0 \\
                             & VSM        & 76.7 & 21.3 & 87.8 & 54.1 \\
        \bottomrule
    \end{tabular}
    \smallskip

    \textit{The performance metrics for the trace links predicted by HGen, the baseline embedding model, and the baseline VSM.}
\end{table}



==> tables/coverage_examples.tex <==
\begin{table}
\centering
\caption{Examples of HGEN documentation that provided concept coverage of the manually constructed documentation.}
\label{tab:software_docs}
  \addtolength{\tabcolsep}{-4pt}
\begin{tabular}{L{.8cm}L{2.5cm}L{5.1cm}}
\hline
\textbf{Project} & \textbf{Manual}& \textbf{HGEN} \\ \hline
Drono- logy & Each individual UAV that is included in a Mission Plan shall have an ordered list of one or more flight routes assigned to it. & Flight Plan Assignment: The system shall enable users to assign flight plans to specific drones in the fleet by selecting a drone identifier and flight plan to link together. This assignment shall be persisted in the data model. \\ \hline
SAFA & I can select an artifact to view more details. & The system shall visually indicate the selection status of artifact nodes when users click to select them, highlighting the nodes in the graph visualization, to enable users to focus on specific artifacts of interest for further analysis. \\ \hline
JOC & As a user, I want to be able to explore and interact with the world & As a user who wants to explore 3D virtual environments, I want to be able to navigate and view a 3D world from a first person perspective so that I can immerse myself in the virtual environment. \\ \hline
\end{tabular}
\end{table}


==> temp.tex <==
 \mdfdefinestyle{MyFrame}{%
    linecolor=gray,
    outerlinewidth=.5pt,
    roundcorner=0pt,
    % innertopmargin=\baselineskip,
    % innerbottommargin=\baselineskip,
    innerrightmargin=6pt,
    innerleftmargin=6pt,
    backgroundcolor=gray!20
}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%%%%%%%%%%%%%% CUSTOM COMMANDS %%%%%%%%%%%%%%
\newcommand{\latinphrase}[1]{\textit{#1}}
\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\newcommand{\smalltt}[1]{{\small\texttt{#1}}}
\newcommand{\citesec}[1]{Section~\ref{sec:#1}}
\newcommand{\citefig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\citealgo}[1]{\textsc{Listing}~\ref{algo:#1}}
\newcommand{\citelisting}[1]{\textsc{Listing}~\ref{lst:#1}}
\newcommand{\citetable}[1]{{Table}~\ref{tab:#1}}
\newcommand{\citedef}[1]{\textsc{Definition}~\ref{def:#1}}

\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash}p{#1}} 


\newcommand{\etal}{\emph{et~al.}\xspace}
\newcommand{\fwname}{\textit{xxx}\xspace}

\newcommand{\MtoH}{\textbf{$[M \rightarrow H]$}\xspace}
\newcommand{\HtoM}{\textbf{$[H \rightarrow M]$}\xspace}

% \newcommand{\jch}[1]{{\textcolor{blue}{#1}}} %blue
% \newcommand{\kd}[1]{{\textcolor{red}{#1}}} %red

% \definecolor{dkgreen}{HTML}{006400}
% \newcommand{\ar}[1]{\textcolor{dkgreen}{#1}} %green
\definecolor{grayhighlight}{rgb}{.65,0.65,0.65}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{LightAmber}{rgb}{0.98,0.89,0.74}
\definecolor{menthol}{rgb}{0.64, 0.98, 0.64}
\newcommand*{\mybox}[2]{\colorbox{#1!30}{\parbox{.98\linewidth}{#2}}}

\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}
\newcommand{\hlt}[1]{{\textcolor{alizarin}{#1}}}%orange
\newcommand{\markphase}{ \CIRCLE}
\hyphenation{autono-mous}
